SoS and Planted Clique: Tight Analysis of MPW Moments at all Degrees and an Optimal Lower Bound at Degree Four

The problem of finding large cliques in random graphs and its "planted" variant, where one wants to recover a clique of size $\omega \gg \log{(n)}$ added to an \Erdos-\Renyi graph $G \sim G(n,\frac{1}{2})$, have been intensely studied. Nevertheless, existing polynomial time algorithms can only recover planted cliques of size $\omega = \Omega(\sqrt{n})$. By contrast, information theoretically, one can recover planted cliques so long as $\omega \gg \log{(n)}$. In this work, we continue the investigation of algorithms from the sum of squares hierarchy for solving the planted clique problem begun by Meka, Potechin, and Wigderson (MPW, 2015) and Deshpande and Montanari (DM,2015). Our main results improve upon both these previous works by showing: 1. Degree four SoS does not recover the planted clique unless $\omega \gg \sqrt n poly \log n$, improving upon the bound $\omega \gg n^{1/3}$ due to DM. A similar result was obtained independently by Raghavendra and Schramm (2015). 2. For $2 < d = o(\sqrt{\log{(n)}})$, degree $2d$ SoS does not recover the planted clique unless $\omega \gg n^{1/(d + 1)} /(2^d poly \log n)$, improving upon the bound due to MPW. Our proof for the second result is based on a fine spectral analysis of the certificate used in the prior works MPW,DM and Feige and Krauthgamer (2003) by decomposing it along an appropriately chosen basis. Along the way, we develop combinatorial tools to analyze the spectrum of random matrices with dependent entries and to understand the symmetries in the eigenspaces of the set symmetric matrices inspired by work of Grigoriev (2001). An argument of Kelner shows that the first result cannot be proved using the same certificate. Rather, our proof involves constructing and analyzing a new certificate that yields the nearly tight lower bound by "correcting" the certificate of previous works.

==> correction-lb-evals.tex <==
\subsection{Moment Method for Correction Eigenvalue Lower Bound}

The following is the main claim for this section.

\begin{lemma}
  \label{lem:cor-eval-lb}
  Let $G \sim G(n,1/2)$.
  Let 
  \[
    r_s(j) = \begin{cases}
    1 & \text{ if $s \sim j$}\\
    -1 & \text{ if $s \not \sim j$}\\
    0 & \text{ if $s = j$}
    \end{cases}\mper
  \]
  Let $r_s^{\tensor 2} \in \R^{\nchoose{2}}$ be the vector with entries $r_s^{\tensor 2}(\{i,j\}) = r_s(i) r_s(j)$.
  Let $V = \Span\{r_s^{\tensor 2} \}_{ s\in [n]}$.
  Let $\Pi_V$ be the projector to $V$.
  With probability at least $1 - O(n^{-10})$ over the sample of $G$,
  \[
    \sum_s (r_s^{\tensor 2})(r_s^{\tensor 2})^\top \succeq \Omega(n^2) \Pi_V\mper
  \]
\end{lemma}

We will need the following graph theoretic machinery for the moment method bound.
\begin{definition}
  Let $G$ be a graph on $[n]$.
  A diamond ribbon $R$ of length $2\ell$ is a graph on vertices $s_1,\ldots,s_\ell, t_1,\ldots,t_\ell, u_1,\ldots,u_{2\ell}, v_1,\ldots,v_{2\ell}$.
  It has edges
  \[
    (s_i, u_{2i}), (s_i, v_{2i}), (u_{2i}, t_i), (v_{2i},t_i), (t_i, u_{2i + 1}), (t_i, v_{2i + 1}), (u_{2i+1}, s_{i+1}),(v_{2i+1},s_{i+1})
  \]
  where addition is modulo $2\ell$.

  A labeled diamond ribbon $(R,F)$ is a a diamond ribbon of length $2\ell$ together with a labeling $F : R \rightarrow G$ of vertices in $R$ with vertices from $G$.
  We insist that for $(x,y) \in R$ an edge that $F(x) \neq F(y)$.

  The labeled diamond ribbon $(R,F)$ is contributing if no element of the multiset $\{(F(x),F(y)) \text{ such that } (x,y) \in R\}$ occurs with odd multiplicity.
  It is \emph{disjoint} if the sets
  \[
    \{F(s_i)\}, \{F(t_i)\}, \{F(u_i)\}_{i \text{ odd}}, \{F(v_i)\}_{i\text{ even}}, \{F(v_i)\}_{i \text{ odd}}, \{ F(v_i) \}_{i \text{ even}}
  \]
  are disjoint.
\end{definition}

\begin{lemma}
  Let $(R,F)$ be a contributing disjoint labeled diamond ribbon of length $2\ell$.
  Then it contains at most $3\ell + O(1)$ distinct labels.
\end{lemma}
\begin{proof}
  By our disjointness assumption, every element of the multiset $\{F(s_i), F(t_i) \}$ must occur with multiplicity at least two and similarly for $\{F(u_i)\}$ and $\{F(v_i) \}$.
\end{proof}



\begin{proof}[Proof of \pref{lem:cor-eval-lb}]
  Note that the matrix $R = \sum_s (r_s^{\tensor 2})(r_s^{\tensor 2})^\top$ has row and column spaces both $V$.
  Note also that it factors as $SS^\top$, where $S$ is the $\nchoose{2} \times n$ matrix whose columns are the vectors $r_s^{\tensor 2}$.
  Thus, it will be enough to show that
  \[
    S^\top S \succeq \Omega(n^2) I \quad \text{w.p. $1 - O(n^{-10})$}
  \]
  where here $I$ is the $n \times n$ identity matrix.

  For this, consider the matrix $S^\top S$ indexed by vertices $s,t \in [n]$.
  It has entries
  \[
    S^\top S (s,t) = \iprod{r_s^{\tensor 2}, r_t^{\tensor 2}}
  \] 
  and in particular,
  \[
    S^\top S (s,s) = \iprod{r_s^{\tensor 2}, r_s^{\tensor 2}} = \nchoose{2}
  \]
  So, zeroing this matrix on the diagonal, it is enough to prove that
  \[
    \Norm{S^\top S - \nchoose{2} I} \leq o(n^2) \quad \text{w.p. $1 - O(n^{-10})$}\mper
  \]
  
  Let $H \seteq S^\top S - \nchoose{2} I$.
  Let $H_{i,j}$ for $i \neq j$ be given by
  \[
    H_{i,j} (s,t) = \begin{cases}
    r_s(i) r_s(j) r_t(i) r_t(j) & \text{ if $s \neq t$}\\
    0 & \text{ otherwise}
    \end{cases}\mper
  \]
  Then $H = \sum_{i \neq j} H_{i,j}$.
  Note that $H_{i,j}(s,t) = 0$ if $i \in \{s,t \}$ or $j \in \{s,t \}$.
  Thus the obvious generalization of \pref{lem:partitioning} to the two-parameter family $H_{i,j}$ applies.
  This gives us a family of matrices $H^1 ,\ldots,H^r$ for some $r = O(\log n)$ and a corresponding family of partitions $(S_1^1,S_2^2,S_3^1,S_4^1,S_5^1,S_6^1),\ldots,(S_1^r,\ldots,S_6^r)$ of $[n]$.

  These will be such that $\sum_{i = 1}^r H^i = H$, and
  \[
    H^i(s,t) = \sum_{(j,k) \in {S_i}'} r_s(j) r_s(k) r_t(j) r_t(k)
  \]
  where ${S^i}' \subseteq S_5^i \times S_6^i$ is the subset giving indices so that the corresponding summand has not occurred in any $i'' < i$.
  We will bound $\E \Tr (H^i)^{2\ell}$ for some $\ell$ to be chosen later.
  Every term in the expansion of this quantity corresponds to a disjoint labeled diamond ribbon of length $2\ell$, and the number of nonzero terms is at most the number of contributing disjoint labeled diamond ribbons.
  So $\E \Tr(H^i)^{2\ell} \leq n^{3\ell + O(1)}$.
  The rest follows by standard manipulations.
\end{proof}


==> optimality.tex <==
\section{Optimality of the Analysis of  the MPW Pseudo Distribution} \label{sec:tightness}
Here we present (a generalization of) an argument due to Kelner that the bound we give on the PSDness of the MPW moments is tight up to logarithmic factors.
The degree four version of this argument appears in informal form in \cite{Bar14}.
\Snote{TODO:write this}


